EnvX: Agentize Everything with Agentic AI

The widespread availability of open-source repositories has led to a vast collection of reusable software components, yet their utilization remains manual, error-prone, and disconnected. Developers must navigate documentation, understand APIs, and write integration code, creating significant barriers to efficient software reuse. To address this, we present EnvX, a framework that leverages Agentic AI to agentize GitHub repositories, transforming them into intelligent, autonomous agents capable of natural language interaction and inter-agent collaboration. Unlike existing approaches that treat repositories as static code resources, EnvX reimagines them as active agents through a three-phase process: (1) TODO-guided environment initialization, which sets up the necessary dependencies, data, and validation datasets; (2) human-aligned agentic automation, allowing repository-specific agents to autonomously perform real-world tasks; and (3) Agent-to-Agent (A2A) protocol, enabling multiple agents to collaborate. By combining large language model capabilities with structured tool integration, EnvX automates not just code generation, but the entire process of understanding, initializing, and operationalizing repository functionality. We evaluate EnvX on the GitTaskBench benchmark, using 18 repositories across domains such as image processing, speech recognition, document analysis, and video manipulation. Our results show that EnvX achieves a 74.07% execution completion rate and 51.85% task pass rate, outperforming existing frameworks. Case studies further demonstrate EnvX's ability to enable multi-repository collaboration via the A2A protocol. This work marks a shift from treating repositories as passive code resources to intelligent, interactive agents, fostering greater accessibility and collaboration within the open-source ecosystem.

==> backend.tex <==

\section{Introduction}\label{sec:intro}

Open-source software repositories contribute countless tools and libraries to the community, yet using them in practice often requires painstaking manual agentization of existing repos, including setting up the environment and running the system. At the same time, the rise of \emph{agentic AI} – AI systems that can act autonomously in complex environments – has opened new possibilities to make software more interactive and self-sufficient. Previously, several studies attempted to agentize open-source repositories. Early works explored containerization and dependency management tools to reproduce environments\cite{boettiger2015docker,collberg2016repeatability}. More recent AI-driven approaches use large language model (LLM)-based coding agents to write installation scripts or Dockerfiles automatically\cite{chen2021codex, qian2023communicative}. 

Although these methods have made important strides, several factors still limit their widespread usage. First, these works typically define the agentization process as \emph{only} the setup of packages, which leaves a large gap with respect to agentic functions. Ignoring other essential components like datasets may lead to a failed agent run.
Second, focusing only on the setup of packages also causes failures in agentization due to the lack of verification, leaving underlying risks unresolved. Moreover, prior works do not imbue the agent with any understanding or communication of its own usage or purpose. These studies stop at installation, without facilitating user interaction post-setup, which limits potential communication and collaboration with other agents.  

In this work, we propose to \textbf{agentize open-source repositories}, i.e., to transform any open-source code repository into an autonomous agent that can configure itself and seamlessly interact with users or other agents. We define \emph{the agentization of an open-source repository} as the process of converting a code repository $R$ into a standalone \emph{repository-agent} with two key capacities: the execution capacity and the agentic interactive capacity. 

\textbf{(i) Execution Capacity}: The agent should automatically prepare the complete execution environment for running the service of the current repository, including \emph{all} components needed to run it. In contrast to previous works that only handle package installation\cite{boettiger2015docker, chen2021codex}, we treat the environment holistically as comprising not just packages and software dependencies, but also any required datasets, external models, drivers, hardware specifications, and even validation data to verify the functionality of the repository agent. 

\textbf{(ii) Agentic Interactive Capacity}: The repository-agent should provide users with an interactive, conversational interface without manual coding, which is based on a deep understanding of $R$’s functionality and usage. This capacity facilitates agentic communication and collaboration between users and other agents, supporting the building of the Agentic Web\cite{yang2025agenticwebweavingweb}. In summary, agentizing a repository turns it into a proactive entity that can both configure itself and interoperate with other agents in solving complex tasks.

In this paper, we introduce a novel framework for agentizing open-source code repositories and address the above limitations. Our main contributions can be summarized as follows.
\begin{itemize}
    \item \textbf{Comprehensive Repository-Agent Definition}: We introduce the repository-agent and the agentic process, which generate agents with two essential capacities: understanding capacity and execution capacity. We build repository agents in an agentic format beyond previous works in this research.
    \item \textbf{Graph-Structured Agentization Process}: We model the construction of repository-agents in a graph-based manner. The environment agentization steps are organized into a directed acyclic graph (DAG) of operations, enabling parallel execution of independent setup tasks, which optimizes both efficiency and cost, and reduces hallucinations brought by long context. Moreover, the graph-based process also makes it easier to provide multi-granularity validation, contributing to a reliable agentization process.
    \item \textbf{Agentizing Tool Integration}: We discuss the limitations of tools in the general agentization process under this scenario, and integrate our specific tool designs into our agentization process. Our experiments show the great potential of our tools in alleviating errors in the results.
    \item \textbf{Agentic Interactive Capacity}: We build the agentic interactive capacity on top of a deep understanding of the given repository, which strongly influences interaction between agents. We build a knowledge base of the repository as part of our process, which equips the repository-agent with a deep understanding of the agentized repository.
\end{itemize}
In the following sections, we detail our methodology for agentizing open-source repositories, first introducing preliminaries in Section 2 and continuing with construction details in Section 3.

\section{Preliminaries}\label{sec:preliminary}

In this section, we formalize the core objectives of our agentization process and provide clear mathematical definitions for introducing our methodology.

\subsection{Graph-Based Agentization Process}\label{subsec:graphprocess}
For a repository $R$, the core part is the setup process, which provides an environment for running the repository-agent. Let $\Sigma$ denote the space of environment states and let $\sigma\in\Sigma$ be the current state. We model the setup process as a directed acyclic graph (DAG):
\[
G_R=(V,E),\quad E\subseteq V\times V,
\]
where vertices $V$ are setup nodes, consisting of a generated target and atomic operations, and edges encode precedence: $(v_a,v_b)\!\in\!E\Rightarrow v_a$ must be completed before $v_b$ begins, and the task in $v_b$ is considered the successor of the task $v_a$. A topological ordering $\pi:V\!\to\!\{1,\dots,|V|\}$ with $\pi(v_a)<\pi(v_b)$ for all $(v_a,v_b)\!\in\!E$ is a valid serial plan; independent nodes can execute in parallel. We may optionally attach positive weights $w:V\!\to\!\mathbb{R}_{>0}$ (durations) and resource demands $d_{v,r}$ for resource types $r\in\mathcal{R}$ with capacities $\kappa_r$.

\subsection{Node}\label{subsec:node}
A node $v\in V$ is a middle step of the setup process, consisting of the following attributes:
\[
v \;=\; \langle g,\; o,\; C,\; S,\; \textsf{pre}_v,\; l \rangle,
\]
where $g$ is the goal of the current node, $o$ is the generated operation, $C$ is the (trajectory-scoped) context usable by the executor, $S\in\{\texttt{pending},\texttt{running},\texttt{done},\texttt{failed}\}$ is the state, $\textsf{pre}_v:\Sigma\!\to\!\{0,1\}$ is the pre-predicate, and $l$ represents the subsequent goals after the current node $\sigma$. The generation process of node $v$ is triggered after the pre-predicate is satisfied, based on the input goal and generated with $f_g$: 
\[
\textsf{pre}_v(\sigma)=1 \;\Rightarrow\; o = f_g(g, C).
\]
Then an operator $f_o$ and a next-step generator $f_l$ are applied to the current state $\sigma$ to generate post-predicates $\sigma'$:
\begin{equation}
\begin{split}
&c \;=\; f_o(o)\\
&C \; = C\; \cup \; c \\
&l \;= f_l(o, C, g) \\  
&\sigma' \;= \sum_{i=1}^n f_g(l_i, C), \quad n=|l|. \\
\end{split}
\end{equation}

\subsection{Trajectory}\label{subsec:trajectory}

A \emph{trajectory} $\in \mathcal{T}(R)$ can be defined as follows:

\[
\tau \; = \langle \; g(\tau),\; P_\tau, \; C_\tau , \; V_\tau \; \rangle
\]

consisting of (i) a goal $g(\tau)$ to be achieved, which is the goal of the root node; (ii) a directed acyclic graph $g(\tau)=[\,v_1\!\to v_2\!\to\cdots\!\to\! v_k\,]$ consisting of nodes, starting with a root node $v_1$; (iii) a trajectory context $C_\tau$ (code/doc slices, commands, configurations); and (iv) a validation set $V_\tau$ to verify the completeness of $g(\tau)$. We generate a trajectory once we obtain a new goal $g_\tau$ and create node $v_{g_{\tau}}$. We treat this node as the root in $P_\tau$ and generate the verification set $V_\tau$.  

\section{Methodology}\label{sec:method}

In this section, we describe our approach to transform a given open-source repository $R$ into a fully functional agent. The process consists of four main components: (1) generating validation data to ensure completeness of the agentization, (2) structuring the environment setup as a graph of operations, (3) integrating real-world tools to carry out setup tasks, and (4) constructing a usage knowledge base for the repository. We explain each component in detail below, along with formal definitions and their benefits.

\subsection{Graph-Structured Agentization Process}\label{sec:graph}
In this section, we propose how we agentize a repository in a graph-structured manner. As introduced in \ref{sec:preliminary}, we define the node and trajectory for the agentization process. As shown in \ref{alg:graph-trajectory}, we first introduce the algorithm to agentize a trajectory with a given repository $R$, context $C$, and the goal of agentization $g$. The core of the graph-structured agentization process is to generate the TODOs for the given goal, and divide them into several sub-trajectories when the goal requires multiple TODOs to achieve. The goals of the newly generated trajectories are set based on the TODOs of the current trajectory. As for the complete agentization of the given repository, we denote the process in \ref{alg:repo-agentization}, where we start only with the repository $R$ and set up the repository goal $g_{repo}$ as \textsc{To agentize the given repo}. We agentize the repository starting with the initialized root node, and also build the repository-level verification data in this step, checking the completeness of agentization when the system reports that all processes have been completed.

As introduced in \ref{sec:intro}, our design has a well-defined acyclic structure, which supports goal-driven expansion from the root $v_g$ to a complete graph. Moreover, the agentization process supports local verification and self-reflection at multiple granularities; the details will be introduced in \ref{sec:validation}.

\begin{algorithm}
\caption{Graph-Structured Agentization for a Trajectory}\label{alg:graph-trajectory}
\begin{algorithmic}[1]
\State \textbf{Input:} Repository $R$; initial trajectory goal $g_\tau$; initial context $C_\tau$.
\State \textbf{Output:} $\tau=\langle g(\tau),\,P_\tau,\,C_\tau,\,V_\tau\rangle$ with $g(\tau)=g_\tau$ and DAG $P_\tau$.

\State $\sigma_\tau, v_{g_\tau} \gets \textsc{InitTrajectory}(R, g_\tau, C_\tau)$
\State $V_\tau \gets \textsc{InitValidationData}(R, g_\tau, C)$
\State $P_\tau \gets (\emptyset,\emptyset)$; \quad $V_\tau \gets \textsc{InitValidation}(R, g_\tau)$
\State Add $v_{g_\tau}$ to $P_\tau$ as root; \quad $Q \gets [\,v_{g_\tau}\,]$

\While{$Q$ not empty}
  \State $v \gets \textsc{PopFront}(Q)$
  \If{$\textsf{pre}_{v}(\sigma)=0$}
     \State \textsc{PushBack}($Q, v$) \Comment{Defer until predecessors/inputs are ready}
     \State \textbf{continue}
  \EndIf

  \State $o \gets f_g(g, C)$ \Comment{Goal $\to$ operation synthesis (using $v$'s goal $g$ \& context $C$)}
  \State $c \gets f_o(o)$ \Comment{Apply operation to produce context increment}
  \State $C \gets C \cup c$; \quad $v.C \gets C$
  \State $l \gets f_l(o, C, g)$; \quad $v.l \gets l$ \Comment{Generate subsequent goals}

  \ForAll{$g' \in l$}
  \State $v' \gets \langle g',\; o=\varnothing,\; C,\; S=\texttt{pending},\; \textsf{pre}_{v'},\; l=\varnothing\rangle$
  \State Add $v'$ to $P_\tau$; \quad Add edge $(v \to v')$ to $P_\tau$
  \State \textsc{PushBack}($Q, v'$)
    \If {$|l|\neq 1$} \Comment{Multiple TODOs, generate new trajectories}
        \State $\tau' \gets \textsc{AgentizationForATrajectory}(R, g', v.C)$
    \EndIf
  \EndFor
  \If {$|l| = 0$} \Comment{No new requirements, start evaluation}
    \State $\sigma' \gets \textsc{Evaluate}(i)$ for $\sum_{i=1}^n$
  \EndIf
  \State $v.S \gets \texttt{done}$
\EndWhile

\State $\sigma_{\tau}^{\text{post}} \gets \sigma$ \Comment{Abstract post-trajectory state}
\If{$\bigwedge_{\phi\in V_\tau}\phi(\sigma_{\tau}^{\text{post}})=1$}
   \State \textbf{Return} $\langle g_\tau, P_\tau, C_\tau, V_\tau\rangle$
\Else
   \State \textbf{Return} $\langle g_\tau, P_\tau, C_\tau, V_\tau\rangle$ with failure status (for external orchestration)
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{algorithm}
  \caption{Repository Agentization}\label{alg:repo-agentization}
  \begin{algorithmic}[1]
    \Require Repository $R$
    \Ensure $\tau=\langle g(\tau),\,P_\tau,\,C_\tau,\,V_\tau\rangle$ with $g(\tau)=g_\tau$ and DAG $P_\tau$

    \State $g_{\text{repo}} \gets \Call{InitRepoTarget}{R}$
    \State $C_{\text{repo}} \gets \varnothing$
    \State $\tau \gets \Call{AgentizationForATrajectory}{R, g_{\text{repo}}, C_{\text{repo}}}$
    \State $V_{\text{repo}} \gets \Call{InitSystemTests}{R}$
    \If{$\sigma_\tau = \text{FINISHED}$}
      \State $\sigma_{\text{repo}} \gets \Call{Evaluate}{V_{\text{repo}}}$
      \If {$\sigma_{\text{repo}} = \text{FINISHED}$}
        \State The agentization is finished.
        \EndIf
      \Else 
        \State \Call{AgentizationForATrajectory}{R, g_{\text{repo}}, C_{\text{repo}}}
     
    \EndIf
  \end{algorithmic}
\end{algorithm}

\subsection{Validation Data Generation for Complete Agentization}\label{sec:validation}

A fundamental challenge in agentizing a repository is ensuring that the resulting agent
works as intended. To address this, our methodology begins by automatically producing a set of \textbf{validation tasks} or \textbf{validation data} $V_R$ for the repository $R$. These validation tasks serve as concrete checks for the completeness and correctness of each trajectory in the agentization process. By having $V_R$ prepared in advance, the agent can verify at the end of each step that the goal is finished as expected, and conduct self-reflection if validation fails.

The generation of $V_R$ can leverage any existing tests or examples in the repository. If the repository already includes a test suite or usage examples, our system will incorporate those into $V_R$. If not, the agent attempts to synthesize validation cases by analyzing the repository’s code and setup goals. We build the $V_\tau$ for each trajectory, and define $V_R=\sum_{i=1}^n V_\tau$ as the union of validation data from all trajectories. Formally, we can view $V_\tau$ as a set of input–output pairs or evaluation queries:
\[
V_\tau \;=\; \{\,(x_i, y_i)\,\}_{i=1}^m,
\]
where each $x_i$ is a generated test instruction or script and $y_i$ is the expected output. The key is that $V_R$ provides an executable test of whether $g_\tau$ has been properly installed and configured.

By generating $V_\tau$ at the start, we set a clear success criterion for the agentization process: the trajectory must be able to pass all tasks in $V_\tau$, and the repository-agent is assumed to be ready only once all $V_R$ checks are passed.

\subsection{Integration of Real-World Tools}\label{sec:tools}

Tools and function calls are widely used in recent agent systems, significantly enhancing the flexibility, scalability, and reliability of agents. In our research, unlike previous systems that issue shell commands or write scripts without truly \emph{understanding} the environment’s state or leveraging existing tools effectively\cite{chen2021codex}, our agentization framework tightly integrates a variety of developer tools and system interactions to align repository agentization with real-world usage.

To align with real-world usage, we design the tools in a human-friendly manner. We build the tools as APIs that provide feedback on success or failure. By integrating real-world tools, we reduce the “sim-to-real” gap: the agent’s operations closely reflect actual environment operations, so state tracking is accurate. This integration also enhances safety by using reliable tools, and reduces hallucinations brought by LLMs. Compared to prior methods that blindly trusted generated scripts, our tool-based approach provides a more governed and robust agentization process.

\subsection{Agentic Communication Capacity}\label{sec:knowledge}

In order to fully agentize a repository, repository-agents require communication and collaboration capacity with users and other agents, which demands a deep understanding of the current repository. For this purpose, we construct a \emph{usage knowledge base} $U(R)$ for each repository $R$ in the agentization process and use it for agentic communication and collaboration.

To build $U(R)$, our system analyzes the source code, documentation, use cases and any metadata (such as README files or docstrings). Using these, the agent extracts key information and structures it into a knowledge base. We can formalize $U(R)$ as a set of usage tuples:
\[
U(R) \;=\; \{\; (q_j,\; a_j) \;\}_{j=1}^n,
\]
where each $q_j$ is a potential agentic request from other agents, and the corresponding $a_j$ is the response. The extraction of $U(R)$ is extended on top of the graph-based agentization (Section~\ref{sec:graph}). After the environment is ready, we add extra nodes that trigger information-gathering actions (like reading the documentation or calling a \texttt{--help} flag). These feed into constructing $U(R)$.

By incorporating a usage knowledge base, our approach ensures that agentization creates a real agent beyond automation of setup. By adding \emph{intelligence} on top of the code, our agentization contributes a self-describing, service-providing agent beyond previous systems, which can strongly support agent infrastructures\cite{yang2025agenticwebweavingweb} in the new era. 

\section{Conclusion}\label{sec:conclusion}
Overall, the methodology we propose results in an agent that can take a raw open-source repository and deliver a fully operational and intelligent service. In later sections, we will showcase examples and case studies of this methodology applied to real repositories, highlighting how each component (validation, graph structuring, tool use, knowledge base) contributes to successful agentization. (The subsequent sections of the paper would contain experiments, discussions, and conclusions accordingly.)

